AI-powered simulation-based inference of a genuinely spatial-stochastic model of early mouse embryogenesis

Understanding how multicellular organisms reliably orchestrate cell-fate decisions is a central challenge in developmental biology. This is particularly intriguing in early mammalian development, where early cell-lineage differentiation arises from processes that initially appear cell-autonomous but later materialize reliably at the tissue level. In this study, we develop a multi-scale, spatial-stochastic simulator of mouse embryogenesis, focusing on inner-cell mass (ICM) differentiation in the blastocyst stage. Our model features biophysically realistic regulatory interactions and accounts for the innate stochasticity of the biological processes driving cell-fate decisions at the cellular scale. We advance event-driven simulation techniques to incorporate relevant tissue-scale phenomena and integrate them with Simulation-Based Inference (SBI), building on a recent AI-based parameter learning method: the Sequential Neural Posterior Estimation (SNPE) algorithm. Using this framework, we carry out a large-scale Bayesian inferential analysis and determine parameter sets that reproduce the experimentally observed system behavior. We elucidate how autocrine and paracrine feedbacks via the signaling protein FGF4 orchestrate the inherently stochastic expression of fate-specifying genes at the cellular level into reproducible ICM patterning at the tissue scale. This mechanism is remarkably independent of the system size. FGF4 not only ensures correct cell lineage ratios in the ICM, but also enhances its resilience to perturbations. Intriguingly, we find that high variability in intracellular initial conditions does not compromise, but rather can enhance the accuracy and precision of tissue-level dynamics. Our work provides a genuinely spatial-stochastic description of the biochemical processes driving ICM differentiation and the necessary conditions under which it can proceed robustly.

==> Manuscript_Organization/Figures_Captions.tex <==
\section*{Figures and captions}

% \graphicspath{{./Manuscript_Graphics/}} % Careful!

% Graphics!

% \section*{Results}

% \subsection*{Multiscale spatial-stochastic model of mouse blastocyst development: from ICM progeny to EPI and PRE lineages}

% Fig~\ref{fig1}.
% \clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 8.75in]{Fig1.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Workflow summary: GRN motif, cell signaling model, and inference framework.} {\bf [A]} The developing ICM is represented by a static spatial lattice of biochemical reaction volumes (cells) coupled via FGF4. Each cell contains a core gene-regulatory network (GRN) featuring mutual repression between the genes \textit{Nanog} (N) and \textit{Gata6} (G), and their self-activation. Both N and G regulate the expression of internal FGF4 (FI). External FGF4 (FE) can either diffuse to a neighboring cell (paracrine signaling), bind to the membrane of the origin cell (autocrine signaling), or be exchanged between neighboring cell membranes. FGF receptors transmit the sensed FGF4 signal back to the core GRN by activating ERK (EI $\leftrightarrow$ EA). {\bf [B]} Pipeline of data generation and analysis. Key stages of parameter inference (columns 1 through 5). Initially, all cells display the undifferentiated (UND) fate (row 2 column 3). Rows 1 and 3 show simulations without and with FGF4 signaling activated, respectively. All generated stochastic trajectories are processed by the same steps: (I) resampling data onto a regular time grid and calculating relevant system observables at cell scale (total NANOG, GATA6, and FGF4 levels); (II) determining the lineage for each cell at every time point (EPI, PRE, or UND); (III) summing up the corresponding total cell count for each fate at tissue scale; (IV) constructing the (joint) pattern score time series. The map between simulation parameters and resultant score time series is used for training a deep neural density estimator via the sequential neural posterior estimation (SNPE) algorithm (row 5 column 5), which directly estimates the parameter posterior distribution (row 5 column 3) conditioned on a target observation (row 4 column 5). Multiple posterior estimates are produced with the same training set, selecting the best learned distribution conditional on the target observation by analyzing a ``meta score'' distribution (row 4 col 3). This summary/meta score is calculated per posterior, and it relies on the maximum a posteriori (MAP) estimate of all the model parameters. In general, the next-round prior does not need to be the current-round posterior: it is plausible to obtain a well-informed next-round mixture distribution (row 5 col 1). Several iterations of the workflow are performed until the meta score surpasses an arbitrarily prescribed level. For additional information about this data-processing pipeline, please see \nameref{subsection:inference_framework}.}
\label{fig1}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Exploring model parameter space via SBI}

% Fig~\ref{fig2}.
% \clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 7.5in]{Fig2.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Summary of inferred central GRN and signaling model parameters (ITWT versus RTM).} Two parameter sets were learned for distinct systems capable of recapitulating the correct final ratio between the emerging ICM lineages (EPI and PRE). The wild-type-like system ITWT (left column) with functional cell-cell signaling via FGF4 (green color), and the mutant-like system RTM (right column) for which FGF4 signaling was inhibited. Black-colored numbers show the inferred values (MAP estimates) of the relevant parameters defining the central intracellular GRN (top row) and the extracellular signaling topology (bottom row) components. Red- and cyan-colored percentage values indicate relative interaction strengths calculated via the formula $\nu = 100(\omega-\theta)/\omega$. Here $\omega$ is the length of the respective parameter range used for the inference scheme, and $\theta$ is the MAP estimate of the particular parameter. Cyan and red colors refer to gene activation and repression, respectively.}
\label{fig2}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{ICM cell-fate differentiation materializes at tissue level}

% Fig~\ref{fig3}.
\clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 7.5in]{Fig3.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Stochastic trajectories at cell and tissue scale.} The ITWT system shows excellent agreement with various experimentally observed characteristics of ICM cell specification. All simulations start with all cells in the undifferentiated (UND) state, having well-balanced cellular resources, before committing exclusively to EPI or PRE fates. {\bf [A]} Example cell-level stochastic trajectory, randomly taken from a 100-cell (10{\texttimes}10 grid) simulation. Within the first 24~h, the cell remains in the UND fate while the FGF4 protein level increases. At around 24~h, a symmetry-breaking event occurs, as the NANOG and GATA6 protein levels take divergent expression paths. Within the last 24~h, the cell acquires the PRE fate while FGF4 levels decrease again. {\bf [B]} Example tissue-level stochastic trajectory of cell fate counts in a 10{\texttimes}10 cell-grid system. Each cell is categorized into one of three possible fates: UND, EPI, or PRE. With progressing time, UND cells reduce in number while EPI and PRE cell counts settle close to prescribed constant target levels (dotted lines); see Methods section \nameref{subsection:computational_experiments} for details of cell-fate classification. {\bf [C]} Typical cell-level behavior of NANOG (blue), GATA6 (orange), and FGF4 (green) total protein levels. {\bf [D]} Typical tissue-level behavior of EPI (blue), PRE (orange), and UND (olive) cell-fate counts. Solid lines represent means, dashed lines represent standard deviations around means. Statistics are computed from a batch of 1000 simulations of a 100-cell tissue system.}
\label{fig3}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{EPI cells precede and are necessary for specification of PRE cells}

% Fig~\ref{fig4}.
% \clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 5in]{Fig4.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf EPI cells precede and are necessary for specification of PRE cells. Expression profiles reveal strong linear correlations among key proteins.} Upper row shows typical cell-level protein count time evolution for each cell-fate category. Cell fates were identified at 48~h. For each fate, cell-level dynamics were traced from last to initial simulation data point. {\bf [A-C]} Solid lines represent mean behavior, dashed lines represent standard deviations around means. Gray regions accentuate time intervals of first differentiated cell appearance for the given fate (vertical dash-dotted line = mean time). Statistics are computed from a batch of 1000 simulations. Only the most relevant proteins are shown: FGF4 (green), NANOG (blue), GATA6 (orange). {\bf [D-F]} Pairwise relationships among the most important proteins at 48~h. Inner panels show different colors representing the protein-pair relationship for the respective cell fate: UND (olive), EPI (blue), PRE (orange). Outer panels show protein count histograms. Data points come from a batch of 1000 simulations. \emph{r\textsubscript{xy}} = Pearson's product-moment correlation coefficient. For details of cell-lineage classification, see Methods section \nameref{subsection:computational_experiments}.}
\label{fig4}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Expression profiles reveal strong linear correlations among key proteins}

% No figure, no caption!

% \subsection*{Intercellular communication noise has key functional advantage: it improves ICM differentiation robustness by 10-20\% compared to purely-binomial baseline scenario}

% Fig~\ref{fig5}.
\clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 7.5in]{Fig5.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Noise at tissue level: intercellular communication improves ICM differentiation robustness by 10-20\% compared to purely-binomial baseline scenario.} {\bf [A]} Comparison between inferred-theoretical wild-type (ITWT $\sim$ CV\textsubscript{1}) and purely-binomial (PB $\sim$ CV\textsubscript{0}) systems. The main plot shows the coefficient of variation (CV) as a function of the system size for each cell fate (colors as in Fig~\ref{fig4}). The inset shows the ratio between CV\textsubscript{0} and CV\textsubscript{1}, highlighting systematically lower fate specification error in the ITWT compared to the PB system. {\bf [C]} Comparison between reinferred-theoretical mutant (RTM $\sim$ CV\textsubscript{1}) and purely-binomial (PB $\sim$ CV\textsubscript{0}) systems. Colors and symbols as in [A]. The inset plot shows that fate specification errors in the spatially uncoupled RTM system are of the same magnitude as in the PB scenario. Axes use logarithmic (base 10) scale. For each system size, the data point is computed from a batch of 1000 simulations. {\bf [B, D]} Typical time evolution of normalized cell fate counts for three example system sizes ($\eta \in [25, 100, 400]$ cells). Solid lines represent means, dashed lines represent standard deviations around means.}
\label{fig5}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Robust cell-fate proportions are independent of cell-grid size}

% No figure, no caption!

% \subsection*{Autocrine- and paracrine-signaling modes play reciprocal roles in robust cell-cell communication}

% Fig~\ref{fig6}.
\clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 1.875in]{Fig6.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Autocrine- and paracrine-signaling modes play reciprocal roles in robust cell-cell communication.} The figure shows the effects of perturbing autocrine- and paracrine-signaling modes in theoretical mutant (TM) systems. {\bf [A]} The TM-APM (inhibition of autocrine, paracrine, and membrane-exchange signaling) represents the loss-of-function phenotype of experimental FGF/ERK pathway mutants. {\bf [B, C]} The complementary TM-A and TM-PM portray the importance of individual feedback modes (paracrine plus membrane exchange and autocrine signaling only, respectively; see also inset text). Solid lines represent mean and standard deviation values ($\mu and \sigma$) for a given TM; dashed lines represent $\mu$ and $\sigma$ for the ITWT. {\bf [D]} Cell-lineage allocation at the 48~h time point. All TMs are compared against the inferred-theoretical wild type (ITWT). For all compared systems, statistics were calculated from 1000 independent simulation runs.}
\label{fig6}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Do ICM cells produce similar local and global neighborhood features? Is the salt-and-pepper pattern a self-similar-like configuration?}

% Fig~\ref{fig7}.
% \clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 3.75in]{Fig7.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Exploring self-similarity and spatial dynamics of simulated ICM neighborhoods.} {\bf [A-C, E-G]} Temporal evolution of spatial correlations among acquired cell fates. Panels [A-C] (upper row) and [E-G] (lower row) show cell-neighborhood degrees 1 and 2, respectively. Here $\rho_{1}$ and $\rho_{0}$ represent mean cell-neighborhood composition values split by fate: $\rho_{1}$ is directly computed from the spatio-temporal distribution of cell fates in ITWT simulations; in contrast, $\rho_{0}$ represents a multinomial baseline model assuming that cell fates emerge in a spatially uncoupled fashion from independent trials leading to acquisition of one of three cell fates with fixed occurrence probability. The latter is estimated by averaging cell fate proportions at every time point across simulations, discarding any spatial information. {\bf [D]} Example of cell neighborhood at 48-h time point. {\bf [H]} Mean and standard deviation of FGF4 protein count as functions of maximum cell-neighborhood degree. FGF4 levels quickly become uncorrelated beyond nearest-neighbor cell distance.}
\label{fig7}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Initial condition noise enhances patterning accuracy and simultaneously sustains its precision}

% Fig~\ref{fig8}.
\clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 7.5in]{Fig8.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Initial-condition variations enhance patterning accuracy and simultaneously sustain its precision.} Robustness to initial-condition perturbations (ICPs): uniform perturbation of protein (NANOG, GATA6) and mRNA (\textit{Nanog}, \textit{Gata6}) initial resources. {\bf [A]} Example initial-condition distributions (ICDs) with increasing variability (see legend) for NANOG and GATA6 proteins (analogous mRNA data not shown for simplicity). Interior scatter plots show sampling intervals; exterior plots show sampling distributions. The 0\% distribution defines the unperturbed baseline case. For each ICD, data points come from 1000 independent simulations. {\bf [B]} Mean cell-fate composition (bars) with standard deviation (error bars) for all tested variability intensities. Bar height ranges from 50 to 100 cells. {\bf [C]} Time trajectories of mean cell-fate counts for selected ICD variability intensities. Dotted lines specify target proportions for EPI and PRE fates, respectively. {\bf [D]} Time trajectories of cell-fate count standard deviations for selected perturbation intensities. Inset plot displays temporal coefficient of variation ($CV = \sigma{\slash}\mu$) for the last 24~h. Colors represent different cell fates. Statistics were calculated from batches of 1000 independent simulations per ICD.}
\label{fig8}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Perturbation buffering is predominantly determined by number of initially affected cells: patterning is robust when less than 25\% of cell population has perturbed initial conditions}

% Fig~\ref{fig9}.
\clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 3.75in]{Fig9.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Resilience to perturbations is mainly determined by number of affected cells: patterning remains robust when less than 25\% of cell population is perturbed.} Robustness to linear initial condition perturbations (ICPs) of protein and mRNA initial resources (NANOG-GATA6 and \textit{Nanog}-\textit{Gata6}). Upper row [A-D] shows the effect of equally perturbing resources of both genes. Lower row [E-H] shows adversarial perturbation of the resources, i.e. linearly progressing perturbation magnitude from 200\% NANOG and 0\% GATA6 (\textminus{100}\% ICP scenario) to 0\% NANOG and 200\% GATA6 (100\% ICP scenario). {\bf [A, E]} Initial condition distributions (ICDs) for NANOG and GATA6 proteins (analogous mRNA distributions not shown for simplicity). Interior (scatter) plots show sampling intervals. Exterior plots show sampling distributions. For each ICD, data points come from 1000 independent simulations. {\bf [B-D, F-H]} Quantifying the effect of equal [B-D] and adversarial [F-H] ICPs for different intensities (molecular count percentage with respect to baseline scenario: ICP = 0\%), and varying number of perturbed cells for all different cell-fate categories (EPI, PRE, UND). For each fate category, color saturation indicates the fate error, i.e. the mean difference of cell-fate counts between the perturbed and unperturbed baseline systems. Each matrix entry (perturbation pair) is calculated from 1000 independent simulations.}
\label{fig9}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Cell plasticity and FGF4-sensitivity are time-window-dependent processes}

% Fig~\ref{fig10}.
% \clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 3.75in]{Fig10.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Robustness to varying amounts of exogenous FGF4 added at distinct time points quantified by SAFD at 48~h: cell plasticity and FGF4 sensitivity are time-window-dependent.} {\bf [A]} Final cell-fate composition (at 48~h) of the inferred-theoretical wild-type (ITWT) system, for all tested FGF4 protein perturbation magnitudes and FGF4 addition at simulation start (0~h). Bar height ranges from 50 to 100 cells. {\bf [B-D]} Effect of different FGF4 perturbation magnitudes and FGF4 addition times on cell-fate composition at 48~h, quantified by Standardized Absolute Fate Deviation (SAFD) for all three fate categories (EPI, PRE, UND) in the ITWT system. SAFD (color represents amplitude) refers to the distance from the reference (or null) configuration (no exogenous FGF4 at 0~h) to every alternative perturbation magnitude and addition time. SAFD is defined as the absolute difference between the mean of reference and perturbed proportions, rescaling this absolute difference by the standard deviation of the reference proportion. The separating hyperplane indicates the boundary between the regions with distance $<= 1$ and distance $> 1$. {\bf [E]} Final cell-fate proportions (at 48~h) of the theoretical mutant system lacking FGF4 production (referred to as TM-FGF4), for all tested FGF4 protein perturbation magnitudes and FGF4 addition at simulation start (0~h). Bar height ranges from 0 to 100 cells. {\bf [F-H]} Effect of different FGF4 perturbation magnitudes and FGF4 addition times on cell-fate composition at 48~h (quantified by SAFD) in the TM-FGF4 system. All bars and data points are calculated from separate batches of 1000 independent simulations for each perturbation.}
\label{fig10}
\end{adjustwidth} % Careful!
\end{figure}

% Fig~\ref{fig11}.
% \clearpage
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 3.75in]{Fig11.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Robustness to varying amounts of exogenous FGF4 added at distinct time points quantified by SAFD at 96~h: cell-fate composition perturbed by non-endogenous FGF4 addition remains largely unchanged beyond 48~h.} {\bf [A]} Final cell-fate composition (at 96~h) of the Inferred-Theoretical Wild-Type (ITWT) system, for all tested FGF4 protein perturbation magnitudes and FGF4 addition at simulation start (0~h). Bar height ranges from 50 to 100 cells. {\bf [B-D]} Effect of different FGF4 perturbation magnitudes and FGF4 addition times on cell-fate composition at 96~h (quantified by SAFD) in the ITWT system. {\bf [E]} Final cell-fate proportions (at 96~h) of the theoretical mutant system lacking FGF4 production (referred to as TM-FGF4), for all tested FGF4 protein perturbation magnitudes and FGF4 addition at simulation start (0~h). Bar height ranges from 0 to 100 cells. {\bf [F-H]} Effect of different FGF4 perturbation magnitudes and FGF4 addition times on cell-fate composition at 96~h (quantified by SAFD) in the TM-FGF4 system. See caption of Fig~\ref{fig10} for definition of SAFD.}
\label{fig11}
\end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Exploring model parameter space via SBI}

% Fig~\ref{fig101}.
\clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 7.5in, height = 7.5in]{Fig101.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Summary of inferred core GRN motif interactions (ITWT versus RTM).} The central component of our inference scheme is the sequential neural posterior estimation (SNPE) algorithm. Both unconditional (top row [A, B]) and conditional (bottom row [C, D]) posterior parameter distributions were obtained following 8 consecutive rounds of inference. 800 thousand composite simulations were performed for the ITWT system (left column [A, C]). For the RTM system (right column [B, D]), 4 consecutive rounds of inference were performed producing 400 thousand simulations. For complete details of the model parameter inference procedure, see \nameref{subsection:inference_framework}. {\bf [A, B]} Model parameter posterior distribution. For ease of visualization, we only show the one-dimensional projection of all posterior components representing the core GRN motif interactions. {\bf [C, D]} First assessment of model parameter sensitivity. These panels show the same components as in [A, B] but the posterior is now conditioned on the maximum-a-posteriori probability (MAP) estimate of the model parameters.}
\label{fig101}
\end{adjustwidth} % Careful!
\end{figure}

% Fig~\ref{fig102}.
\clearpage
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 4.375in, height = 8.75in]{Fig102.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Summary of inferred signaling and other model parameter interactions (ITWT only).} The central component of our inference scheme is the sequential neural posterior estimation (SNPE) algorithm. Both unconditional (top rows [A-D]) and conditional (bottom rows [E-H]) posterior parameter distributions were obtained following 8 consecutive rounds of inference. 800 thousand composite simulations were performed for the ITWT system. For complete details of the model parameter inference procedure, see \nameref{subsection:inference_framework}. {\bf [A-D]} Model parameter posterior distribution. For ease of visualization, the posterior was arbitrarily partitioned into four distinctive groups. We emphasize the top-right group [B, F], which displays the most important signaling model parameter interactions. {\bf [E-H]} First assessment of model parameter sensitivity. These panels show the same components as in [A-D] but the posterior is now conditioned on the maximum-a-posteriori probability (MAP) estimate of the model parameters.}
\label{fig102}
\end{adjustwidth} % Careful!
\end{figure}

% \section*{Materials and methods}

% \subsection*{Computational model of mouse blastocyst (ICM cell differentiation)}

% \subsubsection*{Model at cell scale}

% Fig~\ref{fig103}.
\clearpage
\begin{figure}[hpt!]
% \begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 5in, height = 2.5in]{Fig103.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
% \end{adjustwidth} % Careful!
% \begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Architecture of the modeled gene regulatory region.} Transcription factor (TF) \emph{A} binds to regulatory sites \emph{B} at an effective rate proportional to $k_b$ and unbinds from them at an effective rate proportional to $k_u$. Unlike $k_b$, $k_u$ is directly related to \emph{q} (which is the maximal occupancy of \emph{B} by \emph{A}); i.e., $k_{b,1} = \cdots = k_{b,q}$, where \emph{q} is the number of TF binding sites (TFBSs) for \emph{A} at \emph{B}. {\bf [A]} Markov chain transition diagram of TF binding/unbinding dynamics. {\bf [B]} Every gene has a respective regulatory region with multiple independent binding sites for each of its regulating TFs. Gene activation and repression are both cooperative: exactly \emph{q} TF copies must be simultaneously bound to their particular sites for activation (cyan triangles) or repression (red squares) of expression. By default, repression takes precedence over activation.}
\label{fig103}
% \end{adjustwidth} % Careful!
\end{figure}

% \subsection*{Computational experiments}

% Fig~\ref{fig104}.
% \clearpage
\begin{figure}[hpt!]
% \begin{adjustwidth}{-2.25in}{0in} % Careful!
\includegraphics[width = 5in, height = 2.5in]{Fig104.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
% \end{adjustwidth} % Careful!
% \begin{adjustwidth}{-2.25in}{0in} % Careful!
\caption{{\bf Overview of cell-grid sizes employed for inference and simulations.} The 25-cell grid size (purple highlighting) was used invariably for the actual model parameter inference scheme. All test simulations (assessment of system properties such as robustness in wild-type-like and mutated conditions) employed the 100-cell tissue size (dark-blue highlighting). The remaining cell-grid sizes (gray) were solely used to study tissue-level noise (see also Fig~\ref{fig5}).}
\label{fig104}
% \end{adjustwidth} % Careful!
\end{figure}

\clearpage % Careful!

